An Experimental Survey on Big Data Frameworks

Recently, increasingly large amounts of data are generated from a variety of sources. Existing data processing technologies are not suitable to cope with the huge amounts of generated data. Yet, many research works focus on Big Data, a buzzword referring to the processing of massive volumes of (unstructured) data. Recently proposed frameworks for Big Data applications help to store, analyze and process the data. In this paper, we discuss the challenges of Big Data and we survey existing Big Data frameworks. We also present an experimental evaluation and a comparative study of the most popular Big Data frameworks. This survey is concluded with a presentation of best practices related to the use of the studied frameworks in several application domains such as machine learning, graph processing and real-world applications.

==> mapreduce.tex <==
\section{MapReduce}
\label{sec:mapred}
\subsection{MapReduce Programming Model}


% In this section, we first present the \mapreduce framework and its related concepts. 
% Then, we survey some other Big Data frameworks and we highlight their features. 
% Finally, we provide a categorization of the studied frameworks according to their features. 
% \subsection{\mapreduce framework}
% \subsubsection{System overview}
% \mapreduce is a framework for processing highly distributable problems across huge datasets using a large number of computers. 
MapReduce is a programming model that was designed to deal with parallel processing of large datasets. % with heterogeneous data (i.e., web pages, images, text and sounds) in distributed environments \cite{2li2016heuristics}.
% This model is not new but it is inspired from classical parallel processing. More precisely, it was proposed by Google in 2004.  
MapReduce has been proposed by Google in 2004 \cite{mapreduce} as an abstraction that allows to perform simple computations while hiding the details of parallelization, distributed storage, load balancing and enabling fault tolerance.
% \mapreduce makes the development of programs very easy compared to conventional methods. 
The central features of the MapReduce programming model are two functions, written by a user: Map and Reduce. 
The Map function takes a single key-value pair as input and produces a list of intermediate key-value pairs. 
The intermediate values associated with the same intermediate key are grouped together and passed to the Reduce function. 
The Reduce function takes as input an intermediate key and a set of values for that key. It merges these values together to form a smaller set of values. 
% It consists of dividing each program in two successive phases: Map and Reduce. 
% The Map function takes as input pairs <key, value> to treat and eventually produce intermediate pair under the same structures (<key, value>). 
% The reduce  function collects thereafter, the results issued by the Map function in disks in order to store them in final places representing the final results of treatment \cite{4doulkeridis2014survey}. 
The system overview of \mapreduce is illustrated in Fig.~\ref{fig:mr}. 

\begin{figure}[t]
\centering
\includegraphics[width=0.5\textwidth]{figs/MR.png}
\caption{The MapReduce architecture.}
\label{fig:mr}
\end{figure}

As shown in Fig.~\ref{fig:mr}, the basic steps of a MapReduce program are as follows: 
\begin{enumerate}
\item \textbf{Data reading:} in this phase, the input data is transformed to a set of key-value pairs. 
The input data may come from various sources such as file system, database management system (DBMS) or main memory (RAM). 
The input data is split into several fixed-size chunks. Each chunk is processed by one instance of the Map function.
\item \textbf{Map phase:} for each chunk having the key-value structure, the corresponding Map function is triggered and produces a set of intermediate key-value pairs. 
\item \textbf{Combine phase:} this step aims to group together all intermediate key-value pairs associated with the same intermediate key.
\item \textbf{Partitioning phase:} following their combination, the results are distributed across the different Reduce functions.
\item \textbf{Reduce phase:} the Reduce function merges key-value pairs having the same key and computes a final result. % e.g., a list of key-value pairs. 
% This result is stored in one of the aforesaid storage locations.
% \item \textbf{write the final Results:} The results aggregated by the reduce function will be transferred to the user.
\end{enumerate}


 \subsection{MapReduce challenges}
Although \mapreduce has proven to be effective, it seems that the related programming model is not optimal and generic. 
By studying the literature, we found that several studies and various open source projects are concentrated around MapReduce to improve its performance. 
In this context, challenges around this framework can be classified into two main area: (1) data management and (2) scheduling. 

\textbf{Data management.} 
In order to initiate MapReduce jobs, we need to define data structures and execution workflows in which the data will be processed and managed. 
Formerly, traditional relational database management systems were commonly used. 
However, such systems have shown their disability to scale with significant amounts of data. 
To meet this need, a wide variety of different database technologies such as distributed file systems and NoSQL databases have been proposed \cite{nosql} \cite{gfs}. Nevertheless, the choice of the adequate system for a specific application remains challenging \cite{nosql}.  
%For example, \hadoop \cite{9white2012hadoop} makes use of a distributed file system called \hdfs which is unexpected of distributed file systems pioneered by Google GFS (Google File System). The potential of \hdfs is to enable the processing of large files with different structures.

\textbf{Scheduling.} 
% The \mapreduce framework allows distributed processing over several distributed machines. 
Scheduling is an important aspect of \mapreduce  \cite{scheduling1}. During the execution of a MapReduce job, several scheduling decisions need to be taken. 
These decisions need to consider several information such as data location, resource availability and others. 
For example, during the execution of a MapReduce job, the scheduler tries to overcome problems such as \textit{Map-Skew} which refers to imbalanced computational load among map tasks \cite{mapskew}. 

We notice that minimizing the communication cost is also an important challenge of MapReduce-based applications. 
This communication cost is the total amount of data to be moved from the data storage location to the Mappers and also from the Map phase to the Reduce phase during the execution of a MapReduce job.  
%and maximizes the use of resources. 
%However, \mapreduce scheduler presents some problems that canbe divided into two large families \cite{}: 
%\begin{enumerate}
% \item \textbf{Scheduling in heterogeneous cluster:} an heterogeneous cluster is composed of a set of calculators with various configuration such as operating system and hardware architectures. 
%% When the data chunks are distributed on these nodes, do not return the results to the same time, for this reason that 
%In this context, the scheduler needs to consider the configurations of the computers in the allocation phase in order to avoid \textit{Map-Skew} which refers to imbalanced computational load among map tasks \cite{mapskew}. 
%\item \textbf{Scheduling in multi-user environment:}
% With the origin of \mapreduce the job  are executed one after another in a cluster, every work send  to cluster  will be prossesing in all nodes of cluster  for this program even if its capacity exceeds the processing necessary for this program.
% this strategy is not effective because does not allow optimal use of resources, [24] proposes an algorithm called FAIR is to divide the entire cluster by sub-cluster and dived the scheduler into tow levels, in the most level top planner directs client requests across the cluster with FIFO algorithm, then for each cluster on the second level the scheduler  affect the fonction (map / reduce) in the sub-cluster.
%\end{enumerate}

% In the following, we present some scheduling problems in \mapreduce. % , techniques and algorithms used in literature.
% We consider that scheduling eduler in \mapreduce is an essential compennet  to improve the  performance, it enables to overcome the problems during the execution of task and maximize the use of resources.
% In [21] the authors divided the schedulers problem in  two large families: 
% \begin{enumerate}
%  \item \textbf{Scheduler in heterogeneous cluster:} an heterogeneous cluster is composed of a set of calculators with various configuration such as operating system and hardware architectures. 
% % When the data chunks are distributed on these nodes, do not return the results to the same time, for this reason that 
% In this context, the scheduler needs to consider the configurations of the computers in the allocation phase in order to avoid \textit{Map-Skew} which refers to imbalanced computational load among map tasks \cite{mapskew}. 
% \item \textbf{Scheduler in multi-user environment:}
% with the origin of \mapreduce the job  are executed one after another in a cluster,every work send  to cluster  will be prossesing in all nodes of cluster  for this program even if its capacity exceeds the processing necessary for this program.
% this strategy is not effective because does not allow optimal use of resources, [24] proposes an algorithm called FAIR is to divide the entire cluster by sub-cluster and dived the scheduler into tow levels, in the most level top planner directs client requests across the cluster with FIFO algorithm, then for each cluster on the second level the scheduler  affect the fonction (map / reduce) in the sub-cluster.
% \end{enumerate}

 \subsection{MapReduce-like systems}
 Several systems have been proposed in order to address the challenges of \mapreduce \cite{commapreduce} \cite{twister} \cite{haloop} \cite{datampi} \cite{hadoopplus} \cite{rdma} \cite{dryad}. 
   
In \cite{commapreduce}, the authors proposed ComMapReduce, an extension of \mapreduce that supports communication between Map functions during the execution of a MapReduce job. ComMapReduce is based on a coordinator between the Map functions that uses a shared space to allow communication. 

In \cite{twister}, Twister has been proposed as an extension of MapReduce. The main goal of Twister is to handle iterative MapReduce problems. Twister provides several features such as the distinction between static and variable data, data access via local disks and cacheable MapReduce tasks, to support iterative MapReduce computations. 

HaLoop \cite{haloop} is a modified version of the Hadoop MapReduce that is designed to serve iterative MapReduce applications. HaLoop improves the efficiency of iterative applications by making the task scheduler loop-aware and by adding various caching mechanisms. HaLoop offers a programming interface to express iterative data analysis tasks. 


DATAMPI \cite{datampi} is an extension of MPI to support MapReduce-like computation. DATAMPI abstracts the  key-value communication patterns into a bipartite communication model, which reveals four distinctions from MPI: (1) Dichotomic, (2) Dynamic, (3) Data-centric, and (4) Diversified features. DATAMPI aims to use optimized MPI communication techniques on different networks (e.g. InfiniBand and 1/10GigE) to support MapReduce jobs. 

It is important to mention that other MapReduce-like systems have been proposed such as Dryad \cite{dryad}, Hadoop+ \cite{hadoopplus} and RDMA-Hadoop \cite{rdma}. 

%Ying Yi Bu and all \cite{ref310} \cite{ref410} are  propose another improvement or extension of mapreduce framework, in their work there have to suport the iterative processing of large data. In this study the authors have almost even keep the architecture of mapreduce basic and it add a component allows us to support the iterative computing.
%The mapreduce framework is a tool for allowing us to develop applications in the processing or the tasks will be executed in the same way on the cluster of processor, all in a transparent way to the user, otherwise this Framework supports the communication between cluster resources (CPU, RAM, Disc, ...). However these advantages brought by the large number of implementations of Mapreduce, they remain limited to the management of massive processing of processor only while we have other massive processing such as image processing, video or interactive games that require Processing by means of specific processors (Graphic Processing Unit).
%Therefore, the authors in this work \cite{ref910}  proposed an extension of Mapreduce which supports the processing of graphic nature and to satisfy the programming constraint or the internal architecture of this type of processor.
%Dryad another improvement or extension of mapreduce, this project is created by microsoft in 2007 \cite{ref1010}  to design distributed applications. The concept of Drayad is to build an application as being a graph oriented, with the vertices are the processing steps and the edges represent data flows between vertices. With this microsoft model could improve two sides: (1) no writing or readings  intermediate results in or from the disc compared to that of hadoop, Dryad directly send the results to the functions reduce with the channels.
%(2) since applications can be considered as graphs, it is also possible to have iterative applications.
%\section{other surveys}
%The big data frameworks saw a very important explosion in terms of scientific publications or open source projects mainly in depot github or in the foundation of soft open source apache, this development of tools or solutions big data motivated several researchers to propose Bibliographic studies or reviews of these technologies.
%In this study \cite{ref111} the authors have proposed an in-depth study of major large data projects such as apache spark and aphe hadoop, in which the authors have focused on some architectural aspect such as the mode of deployment and the size of data supported by each Framework and also put emphasis on some aspect link to horizontal and vertical bagability with others like fault tolerance how each framework has to guarantee this property.
%Other problems related to scaling in automated learning algorithms, which motivates authors to propose a large study \cite{ref311} that presents large libraries or tools to implement machine learning solutions for massive data in this the authors have explained and cited some APIs such as mahoot, sparkMLIB, Flink MLIB and others without entering into the details,and in their experimental studies they were limited in the scalability of the machine learning algorithms.
%Other researcher chose the stream mode to present a bibliographic study around this topic, the work of Xiufeng Liu and his co authors \cite{ref211} have designed their studies to present the frameworks big data oriented stream mode and its characteristics and architecture of what It is composed, but without elaboration of an experimental study and without recommendation of some frameworks for certain use cases.
